Effect of Adaptive and Cooperative Adaptive Cruise Control on Throughput of Signalized Arterials

The paper evaluates the influence of the maximum vehicle acceleration and variable proportions of ACC/CACC vehicles on the throughput of an intersection. Two cases are studied: (1) free road downstream of the intersection; and (2) red light at some distance downstream of the intersection. Simulation of a 4-mile stretch of an arterial with 13 signalized intersections is used to evaluate the impact of (C)ACC vehicles on the mean and standard deviation of travel time as the proportion of (C)ACC vehicles is increased. The results suggest a very high urban mobility benefit of (C)ACC vehicles at little or no cost in infrastructure.

==> 2 - Copy/acc_cacc.tex <==
We will now explore the impact of ACC and CACC vehicles on intersection
throughput.
To do that, we repeat two experiments described in
Section~\ref{sec_intersection_throughput}  but this time,  with a mix of ordinary 
(manually driven), ACC and CACC vehicles.
Values of car following parameters for the three vehicle types
are given in Table~\ref{tab-params-per-vehicle-type}.
As one can see, ACC and CACC vehicles can maintain shorter distances
to the vehicle in front.
%\vspace*{-5pt}
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Vehicle type & $\tau$ (seconds) & $g_{\min}$ (meters)\\
\hline
Ordinary & 2.05 & 4 \\
ACC-enabled & 1.1 & 3 \\
CACC-enabled & 0.8 & 3 \\
\hline
\end{tabular}
\end{center}
\caption{Values of reaction time $\tau$ and minimal gap $g_{\min}$
for ordinary, ACC- and CACC-enabled vehicles.}
\label{tab-params-per-vehicle-type}
\end{table}

We assume that the ACC vehicle has the same car following model as that of the
ordinary vehicle, but with different $\tau$ and $g_{\min}$.  A
CACC vehicle behaves like an ACC vehicle if
it follows an ordinary vehicle, but if it has another CACC car in front,
it assumes different car following behavior, which we call
\emph{CACC car-following model}.

Let $a_{IIDM}(t)$ denote the acceleration function defined by~\eqref{eq_iidm}.
Define the \emph{constant-acceleration heuristic (CAH)} acceleration 
function~\cite{treiberkesting_book}:
\begin{eqnarray}
&& a_{CAH}(t) = \nonumber \\
&& \left\{\begin{array}{l}
\frac{v^2(t)\bar{a}_l(t)}{v_l^2(t)-2(x_l(t)-x(t)-l)\bar{a}_l(t)}, \\
\mbox{ if } \frac{v_l(t)(v(t) - v_l(t))}{2 \bar{a}_l(t)}\leq (x(t)+l-x_l(t));\\
\bar{a}_l(t) - \frac{(v(t)-v_l(t))^2\Theta(v(t)-v_l(t))}{2(x_l(t)-x(t)-l)},
\mbox{ otherwise,}
\end{array}\right.
\label{eq_a_cah}
\end{eqnarray}
where
\[ \bar{a}_l(t) = \min\left\{\dot{v}_l(t), a_{\max}\right\}, \]
and
\[
\Theta(z) = \left\{\begin{array}{ll}
1, & \mbox{ if } z \geq 0,\\
0, & \mbox{ otherwise}.
\end{array}\right.
\]
We now specify the CACC car following
model~\cite{treiberkesting_book}:
\begin{eqnarray}
&& a_{CACC}(t) = \nonumber \\
&& \left\{\begin{array}{ll}
a_{IIDM}(t), \mbox{ if } a_{CAH}(t) \leq a_{IIDM}(t), \\
a_{CAH}(t) + \\
b\tanh\left(\frac{a_{IIDM}(t)-a_{CAH}(t)}{b}\right),
\mbox{ otherwise.}
\end{array}\right.
\label{eq_cacc_model}
\end{eqnarray}

As before, we run the free road and the red light downstream experiments.
For both scenarios we compute the intersection throughput,
when portion of ACC (CACC) vehicles in the initial queue.
Thus we evaluate 24 cases, each defined by:
(1) experiment: free road or red light downstream;
(2) ACC or CACC; and
(3) percentage of ACC (CACC): 10,
25, 50, 75, 90 and 100\%.

Fig.~\ref{fig-acc-portion-free} and~\ref{fig-acc-portion-stop} compare
flows, gaps, speeds and acceleration obtained at the detector location
for 0, 50 and 100\% ACC (CACC) penetration rate.
Three horizontal red lines on flow plots in both figures correspond
to equilibrium flows with 0\% ACC (CACC), with 100\% ACC and with
100\% CACC penetration rate.
These flows are computed as $3600/\theta_e$, where $\theta_e$ is given
by~\eqref{eq_min_headway} with $\tau$ and $g_{\min}$ from
Table~\ref{tab-params-per-vehicle-type}, yielding 1440, 2400 and 3000
vehicles per hour respectively.
In the flow and distance to leader plots, notice how 50\% ACC plots
jump between the no ACC and 100\% ACC plots: for an ordinary vehicles
it is similar to the no ACC curve, and for an ACC vehicle it is
similar to 100\% ACC curve.
50\% CACC curves in the same plots jump between three curves --- no ACC,
100\% ACC and 10\% CACC.
This is because a CACC vehicle following an ordinary one behaves
like ACC vehicle. 
\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/acc_portion_free.pdf}
\caption{Case with free road ahead: comparison of  measurements of flow,
distance to leader, speed, and acceleration at the detector location
for different proportions of ACC/CACC traffic.}
\label{fig-acc-portion-free}
\end{figure}
\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/acc_portion_stop.pdf}
\caption{Case with red light downstream: comparison of point measurements of flow,
distance to leader, speed and acceleration at the detector location
for different proportions of ACC/CACC traffic.}
\label{fig-acc-portion-stop}
\end{figure}

For an ACC (CACC) penetration rate less than 100\%, the intersection
throughput is sensitive to the distribution of ACC (CACC) vehicles
in the initial queue.
For example, if 25\% all vehicles in the initial queue are ACC-enabled,
and all of them are concentrated at the head of the queue, we would get
higher vehicle count at the detector location after one minute, than
we would with 50\% ACC penetration rate when all ACC-enabled vehicles are
concentrated at the tail of the queue.
In another example, 50\% CACC penetration rate would not produce any gain
over 50\% ACC penetration rate, if ordinary and ACC/CACC vehicles were
interleaved--- one ordinary, one ACC/CACC, one ordinary, and so on --- since an
CACC achieves a shorter headway than  ACC only when it has other CACC vehicles directly in front.

To mitigate this ACC (CACC) distribution bias, in each case with
ACC (CACC) penetration rate less than 100\%, we run 100 random one-minute simulations
of the three car-following models, record vehicle counts at the
detector location, and plot the median vehicle count.
For 100\% penetration rate the ACC (CACC) distribution is trivial, and hence,
a single simulation for each case is enough.
The intersection throughput results for all the 24 cases,
together with throughput values from Table~\ref{tab-model-throughput} obtained
for 0 ACC (CACC) penetration rate, are presented as the four plots in
Fig.~\ref{fig-acc-cacc-per-model}.
\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/acc_cacc_per_model.pdf}
\caption{Intersection throughput as a function ACC (top) or CACC (bottom)
portion of traffic computed with IIDM for free
road downstream (left) and red light downstream (right).}
\label{fig-acc-cacc-per-model}
\end{figure}

Note that in each of the four plots in Fig.~\ref{fig-acc-cacc-per-model},
there is a curve corresponding to the \emph{equilibrium} traffic flow.
These equilibrium curves are computed as follows.
Denote by $\lambda\in[0,1]$ the fraction of ACC (CACC) vehicles in the initial queue, and by
$\tau^{[C]ACC}$ and $g_{\min}^{[C]ACC}$ the reaction time and minimal
gap for ACC (CACC) vehicles, whose values are given in
Table~\ref{tab-params-per-vehicle-type}.
The average headway in the equilibrium state is obtained by modifying
expression~\eqref{eq_min_headway}:
\begin{eqnarray}
\theta(\lambda) & = & \lambda \tau^{[C]ACC} + (1-\lambda)\tau + \nonumber \\
& & \frac{\lambda g_{\min}^{[C]ACC} + (1-\lambda)g_{\min} + l}{v_{\max}}.
\label{eq_modified_headway}
\end{eqnarray}
Then, the equilibrium flow in vehicles per minute is given by:
\be
f(\lambda) = 60/\theta(\lambda).
\label{eq_modified_max_flow}
\ee
This formula is sufficient for the case when there is a free road ahead.
In the case of a red light downstream, however, we are restricted
by the capacity of the link connecting the two intersections.
To account for that, we modify~\eqref{eq_modified_max_flow} accordingly:
\begin{eqnarray}
f(\lambda) & = & \min\Big{\{}\frac{60}{\theta(\lambda)}, \nonumber \\
& & \frac{k\Delta}{\lambda g_{\min}^{[C]ACC} + (1-\lambda)g_{\min}+l}\Big{\}},
\label{eq_modified_max_flow2}
\end{eqnarray}
where $\Delta$ is the length of the link between the two intersections,
and $k$ is the number of lanes in that link.
In our experiment, $\Delta = 300$, and $k=1$.





==> 2 - Copy/cfm.tex <==
We start with the notation  in Table~\ref{tab-micro-notation},
and the default parameter values that we will use.
The state  equations for the IIDM car-following model are:
\begin{eqnarray}
v(t+\Delta t) & = & v(t) + a(t)\Delta t ; \label{eq_vehicle_speed}\\
x(t+\Delta t) & = & x(t) + v(t)\Delta t + \frac{a(t)\Delta t^2}{2}.
\label{eq_vehicle_position}
\end{eqnarray}
The critical control variable is acceleration $a(t)$, set by
\begin{eqnarray}
&& a(t) = \nonumber \\
&& \left\{\begin{array}{l}
a_{\max}\left(1-\left(\frac{g_d(t)}{g(t)}\right)^{\delta_1}\right),
\mbox{ if } \frac{g_d(t)}{g(t)} > 1;\\
a^\ast(t)\left(1-
\left(\frac{g_d(t)}{g(t)}\right)^{\frac{\delta_1 a_{\max}}{a^\ast(t)}}\right),
\mbox{ otherwise,}
\end{array}\right.
\label{eq_iidm}
\end{eqnarray}
where
\begin{eqnarray}
a^\ast(t) & = & a_{\max}\left(1-
\left(\frac{v(t)}{v_{\max}}\right)^{\delta_2}\right),
\label{eq_iidm_afree}\\
g_d(t) & = & g_{\min} + \max\Big{\{}0, \nonumber\\
&&  v(t)\tau +
\frac{v(t)(v(t)-v_l(t))}{2\sqrt{a_{\max}b}}\Big{\}},\label{eq_iidm_desired_gap}
\end{eqnarray}
and $\delta_1, \delta_2$ are  fixed positive parameters.
We use $\delta_1=4$, $\delta_2=8$.
The equilibrium speed ($a(t)=0$)
is given by $v(t) = v_l(t) = v_{\max}$
and $g(t) = g_{\min} + v(t)\tau$, and then
the equilibrium headway is
\be
\theta_e = \tau + \frac{g_{\min} + l}{v_{\max}}.
\label{eq_min_headway}
\ee
The default values from Table~\ref{tab-micro-notation} give $\theta_e=2.5$ s,
which translates to $f_e=1/\theta_e=0.4$ vehicles per second, 24 vehicles per minute,
or 1440 vph. Empirical estimates of throughput vary between 1200 and 1900 vph.


\vspace*{-5pt}
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
Symbol & Description &  \begin{tabular}{@{}l@{}}Default\\ 
value\end{tabular}\\
\hline
$l$ & Vehicle length. & $5$ m\\
$t$ & Time. & \\
$\Delta t$ & Model time step. & $0.05$ s\\
$x(t)$ & Vehicle position. &\\
$x_l(t)$ & Position  of the lead vehicle.&\\
$v_{\max}$ & Speed limit. & $20$ m/s\\
$v(t)$ & Vehicle speed. &\\
$v_l(t)$ & Speed of the leader. &\\
$a(t)$ & Vehicle acceleration. &\\
$a_{\max}$ & Maximal vehicle acceleration. & $1.5 \mbox{ m/s}^2$ \\
$b$ & Desired vehicle deceleration. & $2 \mbox{ m/s}^2$\\
$g(t)$ & \begin{tabular}{@{}l@{}}Gap: distance from the front\\
of the vehicle to the tail of the\\
leader,
$g(t)=x_l(t)-x(t)-l$.\end{tabular} &\\
$g_{\min}$ & Minimal admissible gap. & $4$ m\\
$g_d(t)$ & Desired gap. & \\
$\tau$ & Reaction time. & $2.05$ s\\
$\theta(t)$ & Headway: $\theta(t) = \frac{x_l(t)-x(t)}{v(t)}$. &\\
$f(t)$ & Vehicle flow: $f(t) = \frac{1}{\theta(t)}$. &\\
\hline
\end{tabular}
\end{center}
\caption{Notation summary.}
\label{tab-micro-notation}
\end{table}





\section{Intersection Throughput}\label{sec_intersection_throughput}
We analyze the urban arterial of Fig.~\ref{fig-basic-experiment} with infinitely many vehicles in the queue with  minimal gap between them.
At time $t=0$, the light turns green, and vehicles are released. We  discuss two experiments --- one with free road ahead, and the second  with a red light 300 m 
downstream at the second intersection.  This distance accommodates 33 vehicles in the queue
(see Table~\ref{tab-micro-notation} for default values of the car length $l$   and the minimal gap $g_{\min}$), which exceeds the number that
can be sent from the first signal in one minute.
\begin{figure}
\centering
\includegraphics[width=3.2in]{figures/BasicExperiment.png}
\caption{Signal turns green at time $t=0$, and vehicles start
moving.
In the first experiment, the first vehicle has free road ahead.
In the second experiment, the first vehicle encounters red light
at the next intersection, 300 meters downstream.}
\label{fig-basic-experiment}
\end{figure}

Fig.~\ref{fig-trajectories} displays trajectories, speeds and accelerations of the first ten vehicles from the queue  for these two experiments.
The signal is located at position 0 and indicated by the horizontal black line in the top three trajectory plots.
The leader of the first vehicle is infinitely far ahead.  In the experiment with free road downstream, it accelerates with $a^\ast(t)$
from equation~\eqref{eq_iidm_afree}, asymptotically approaching the maximum speed.
In the second experiment with the red light  at position $x_s=300$, a``blocking vehicle'' is placed at position
$ x_b = x_s + g_{\min} + l $ = 300 + 4 + 5 = 309,
with velocity $v_b=0$, which causes the first vehicle to stop at  $x_s$ to maintain the minimal gap.


\begin{figure}
\centering
\includegraphics[width=3.2in]{figures/trajectories.png}
\caption{Vehicle trajectories, speeds and accelerations:
experiment with free road ahead (left); and
experiment with red light ahead (right).}
\label{fig-trajectories}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/ModelComparison.pdf}
\caption{Experiment with a free road ahead: comparison of 
measurements of flow, distance to leader, speed and acceleration
at the detector location between the three car following models.}
\label{fig-model-comparison}
\end{figure}

As a queue builds up in front of  the red light, vehicles slow down, and thereby 
reduce the vehicle flow though the
first intersection.
In the experiment with the red light downstream we study the impact of this
braking effect on the throughput of the first intersection.  (This is the second limitation noted in \cite{platoons}.)

The most interesting for the intersection throughput assessment is the traffic behavior at the stop bar location indicated in Fig.~\ref{fig-basic-experiment}.
Fig.~\ref{fig-model-comparison} presents the  measurements obtained from this detector, with each dot corresponding to a vehicle passing the detector.
The (instantaneous) flow (top left) is computed for a vehicle passing the detector based on the
time elapsed after the previously detected vehicle, taken as a headway $\theta(t)$, which is then inverted ($f(t) = 1/\theta(t)$)
and expressed in vph. The red horizontal line corresponds to the equilibrium flow of 1440 vph in our case, when vehicles move at maximal speed.
The gap (top right) between vehicles as well as the speed (bottom left) are monotonically increasing, while acceleration (bottom right) is monotonically decreasing.

In the case of free road downstream, 23 vehicles cross the intersection during the first minute, slightly below the equilibrium flow
of 24 vehicles per minute. The IIDM control can be tuned to a more aggressive behavior by increasing
its parameters $\delta_1,\delta_2$.  In the case of red light downstream, the flow is reduced to 21 vehicles
during the first minute as the result of braking propagation.

We now examine how throughput at the first intersection in our
two previous experiments depends on the maximal acceleration $a_{\max}$.
We repeat both experiments, with the free road and with the red light ahead,
for three different values of $a_{\max}$: $0.8$, $1.5$ (our default) and  $2.5 \mbox{ m/s}^2$.
Fig.~\ref{fig-acceleration-comparison} presents the  measurements obtained at the stop bar location for the cases of free road (left)
and red light downstream (right).
Table~\ref{tab-model-throughput} summarizes the throughput results
for different acceleration values.  The results for this `base' case will be compared with the increased throughput using (C)ACC.

\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/AccelerationComparison.png}
\caption{Comparing flows for different values of $a_{\max}$
for  experiments  with the free road (left), and
with the red light ahead (right).}
\label{fig-acceleration-comparison}
\end{figure}

\vspace*{-5pt}
\begin{table}[h]
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Value of $a_{\max}$ & Type of experiment & IIDM \\
\hline
\multirow{2}{*}{$0.8\mbox{ m/s}^2$} &
free road ahead & 20 \\
 & red light ahead & 19 \\
\hline
\multirow{2}{*}{$1.5\mbox{ m/s}^2$} &
free road ahead & 23 \\
& red light ahead & 21 \\
\hline
\multirow{2}{*}{$2.5\mbox{ m/s}^2$} &
free road ahead & {\bf 24} \\
& red light ahead & 22 \\
\hline
\end{tabular}
\end{center}
\caption{Summary of  experiments: intersection
throughput in vehicles per minute.
Values equal to the equilibrium flow are  in bold.}
\label{tab-model-throughput}
\end{table}



==> 2 - Copy/conclusion.tex <==
Presence of (C)ACC-enabled vehicles in the traffic increases the
intersection throughput and reduces travel time at all levels of penetration.
CACC vehicles forming a sequence  increase the throughput of an intersection
significantly more than can be achieved with pure ACC vehicles;  but
 CACC vehicles interleaved with ordinary ones have the same effect
as  ACC vehicles.
Queues in short links do reduce the throughput at an upstream intersection.

In an urban network the presence of (C)ACC vehicles reduces the queues and hence
the time spent at intersections.  As a result ordinary as well as (C)ACC vehicles benefit from
lower average travel times with a lower standard deviation.  The results of this paper together with those  in \cite{platoons}
indicate that (C)ACC can greatly improve urban road mobility at little or no additional infrastructure cost.


==> 2 - Copy/iidm_boxplot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
unbounded coords=jump,
xmin=0.5,
xmax=4.5,
xtick={1,2,3,4},
xticklabels={{0},{25},{50},{75}},
ymin=340.16,
ymax=3588.24,
axis background/.style={fill=white}
]
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	3042.5\\
1	3440.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	2414.4\\
2	2712.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	1976.85\\
3	2212.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	1365.45\\
4	1556.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	694.3\\
1	1593.1\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	653.9\\
2	1440.55\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	625.7\\
3	1206.4\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	487.8\\
4	798.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	3440.6\\
1.125	3440.6\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	2712.3\\
2.125	2712.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	2212.3\\
3.125	2212.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	1556.3\\
4.125	1556.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	694.3\\
1.125	694.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	653.9\\
2.125	653.9\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	625.7\\
3.125	625.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	487.8\\
4.125	487.8\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.75	1593.1\\
0.75	3042.5\\
1.25	3042.5\\
1.25	1593.1\\
0.75	1593.1\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
1.75	1440.55\\
1.75	2414.4\\
2.25	2414.4\\
2.25	1440.55\\
1.75	1440.55\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
2.75	1206.4\\
2.75	1976.85\\
3.25	1976.85\\
3.25	1206.4\\
2.75	1206.4\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
3.75	798.7\\
3.75	1365.45\\
4.25	1365.45\\
4.25	798.7\\
3.75	798.7\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.75	2406.3\\
1.25	2406.3\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
1.75	2008.5\\
2.25	2008.5\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
2.75	1584.7\\
3.25	1584.7\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
3.75	1106.7\\
4.25	1106.7\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\end{axis}
\end{tikzpicture}%

==> 2 - Copy/iidm_boxplot_npltn.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
unbounded coords=jump,
xmin=0.5,
xmax=4.5,
xtick={1,2,3,4},
xticklabels={{0},{25},{50},{75}},
ymin=370.82,
ymax=3586.78,
axis background/.style={fill=white}
]
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	3042.5\\
1	3440.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	2653.75\\
2	2901.8\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	1978.85\\
3	2355.5\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	1590.6\\
4	1751.7\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	694.3\\
1	1593.1\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	642.1\\
2	1457.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	517\\
3	1218.15\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	547.2\\
4	895.1\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	3440.6\\
1.125	3440.6\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	2901.8\\
2.125	2901.8\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	2355.5\\
3.125	2355.5\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	1751.7\\
4.125	1751.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	694.3\\
1.125	694.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	642.1\\
2.125	642.1\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	517\\
3.125	517\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	547.2\\
4.125	547.2\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.75	1593.1\\
0.75	3042.5\\
1.25	3042.5\\
1.25	1593.1\\
0.75	1593.1\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
1.75	1457.6\\
1.75	2653.75\\
2.25	2653.75\\
2.25	1457.6\\
1.75	1457.6\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
2.75	1218.15\\
2.75	1978.85\\
3.25	1978.85\\
3.25	1218.15\\
2.75	1218.15\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
3.75	895.1\\
3.75	1590.6\\
4.25	1590.6\\
4.25	895.1\\
3.75	895.1\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.75	2406.3\\
1.25	2406.3\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
1.75	2085.8\\
2.25	2085.8\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
2.75	1628.75\\
3.25	1628.75\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
3.75	1201.05\\
4.25	1201.05\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\end{axis}
\end{tikzpicture}%

==> 2 - Copy/intersection_throughput.tex <==


\subsection{Baic Experiment: Single Intersection}\label{subsec_basic}




\subsection{Effect of the Downstream Queue}\label{subsec_queue_effect}








For vehicles traveling at constant speed with a uniform space headway, the observed throughput per hour is inversely proportional to the reaction time. In particular, for vehicles moving at 20 m/s and a reaction time of 2.5 s (equivalent to a space headway of 2.5 $\times$ 20 = 50 m), a saturation flow rate of 3600/2.5 = 1440 vph is achieved, hereinafter referred to as the steady-state throughput. (cite platoons of connected vehicles... varaiya 2015) \\

With the introduction of a traffic signal and the build-up of a large queue of vehicles, the instantaneous throughput of vehicles can be measured by recording the time headway between successive vehicles. For a sufficiently long green signal in the outbound direction, the time headway of the vehicles is expected to converge to the steady-state equilibrium and the steady-state throughput is believed to be an upper bound on the total flow achievable. However, in simulation it was observed that the total throughput in fact exceeded the steady-state throughput. This was contingent on factors that the steady-state calculations do not consider, such as the rate of acceleration and deceleration of the vehicles. When the signal turns green, the first few cars are packed together due to their accelerating behavior and are not as widely spaced as the cars further in the queue when they approach the intersection. As a result, the observed time headway is less than the steady-state reaction time and an increased throughput is observed.\\

Different scenarios were considered with varying accelerations as well as varying red clear times between switching green signals. The instantaneous throughput for each scenario was plotted and compared to the steady-state theoretical. 


\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/init.jpg}
\caption{Simulation set up with large queues in the North and West lanes both traveling East.}
\label{fig:init}
\end{figure}

Figure \ref{fig:init} shows a picture of the simulation in SUMO. The parameters used were $\theta_{\min} = 2.5$ s with $g_{\min} = 4$ m, $l = 5$ m, $v_{\max} = 20$ m/s, and $\tau = 2.05$ s.  

The first parameter investigated was the affect of signal length. Two different signal plans were used: a one minute cycle and a two minute cycle, each with identical red clear times. For example, a three second red clear time for a two minute cycle would result in the following signal pattern: 57 seconds of EW green, 3 second of all red, 57 seconds of NS green and 3 seconds of all red. This implies that for a one minute cycle, double the red clear time is experienced compared to the two minute cycle for simulations that are integer multiples of two minutes in length. 

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_a15.png}
\caption{Comparison of timing plans for the scenario highlighted in Figure \ref{fig:init} with a red clear time of 3 seconds and acceleration equal to $1.5$ m/s$^2$. The troughs in the curves represent the transition between the last car from the East and the first car in the North and vice versa.}
\label{fig:cycles}
\end{figure}


Although a total decrease in throughput is expected for the one minute cycle, the total throughput in both scenarios highlighted in figure \ref{fig:cycles} was 1440 vehicles after one hour of simulation. This indicates the loss in throughput experienced by more frequently changing timing plans (and consequently more troughs) was balanced out by the high throughput experienced initially after the signal turned green in each direction. Despite this, the total throughput experienced after one hour was equivalent to the steady-state throughput. With a red clear time of 0 seconds, the total throughput observed for the same scenarios were \textbf{ XXXXXXXXXXX} for the one minute and two minute cycles respectively. This implies, paradoxically, that the introduction of a traffic signal in the presence of a seemingly infinite queue can increase the throughput beyond the steady-state bound. \\


The next parameter examined was the maximum acceleration of the vehicles. For vehicles that were not at the front of the queue, their speeds were dictated by (3) whereas the speed of the vehicle at the front of the queue was governed by simple kinematics: $v(t+\Delta t) = v(t) + a\Delta t$ \textbf{(not sure how to cross reference between tex files for equations)} Consequently, the acceleration of the lead vehicle was directly correlated with the speed of its followers - a larger acceleration implied that the following vehicles were able to travel faster as well. As a result, the instantaneous throughput and total throughput observed were larger for the scenarios with higher accelerations. Figure \ref{fig:diffa} compares varying accelerations and the resulting throughputs.\\

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_diffa.png}
\caption{Comparison of accelerations for the scenario highlighted in Figure \ref{fig:init} with a red clear time of 3 seconds and a two minute cycle. The total throughput after one hour for $a = 1.0,\  1.5,\  2.6$ m/s$^2$ was 1380, 1440 and 1510 vehicles respectively.}
\label{fig:diffa}
\end{figure}



Finally, the duration of the red clear time was also experimented with. Increasing the red clear time would predictably decrease the total throughput and increase the size of the troughs in the throughput plots. 

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_diffRCT.png}
\caption{Comparison of red clear times for the scenario highlighted in Figure \ref{fig:init} with a two minute cycle.}
\label{fig:diffRCT}
\end{figure}

In Figure \ref{fig:diffRCT} it is clear that the decrease in throughput between a red clear time of 0 seconds and 3 seconds is much larger than that between 3 seconds and 5 seconds.\\

Although this provides insight into the dynamics of the cars, it is an idealized scenario. As in most urban settings, there is often another signal further downstream, leading to the formation of another queue between the two intersections. This congestion effect significantly decreases the throughput through the first intersection and is correlated with the distance between the two intersections. Figures \ref{fig:100m} and \ref{fig:500m} plot the instantaneous throughput through the first intersection in the presence of a downstream intersection that is 100m and 500m away respectively. The timing plan of the second intersection flipped the order of the green waves. Although the order of the second timing plan is arbitrary, the total throughput will be the same.\\

\textbf{(not sure if graph for 100m is totally correct - had teleporting issues, cite source about how long between intersections in urban setting)}

\begin{figure}[htb!]
\centering
\includegraphics[width=5in]{figures/100m.png}
\caption{Throughput in the presence of downstream intersection 100m away.}
\label{fig:100m}
\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=5in]{figures/500m.png}
\caption{Throughput in the presence of downstream intersection 500m away.}
\label{fig:500m}
\end{figure}

For the 100m and 500m downstream intersections, the total throughput after an hour was 753 and 772 vehicles for zero seconds of red clear time and 722 and 742 vehicles for three seconds of red clear time respectively. For the secondary intersection 100m away, although the peak is much closer to the steady-state theoretical compared to the 500m scenario, its trough is much larger. Because of this, the throughput experienced on average for the 500m scenario is in fact larger as is expected. 

%\begin{figure}
%\centering
%\begin{minipage}{.7\textwidth}
%  \centering
%  \includegraphics[width=.8\linewidth]{figures/100m.png}
%  \captionof{figure}{A figure}
%  \label{fig:test1}
%\end{minipage}%
%\begin{minipage}{.7\textwidth}
%  \centering
%  \includegraphics[width=.8\linewidth]{figures/500m.png}
%  \captionof{figure}{Another figure}
%  \label{fig:test2}
%\end{minipage}
%\end{figure}


This, in conjunction with the results of varying acceleration and timing plans, poses further questions: for a given acceleration, what is the optimal signal length and red clear time to maximize the number of cars that can pass through an intersection? Is it more advantageous to have short bursts in cycles to solely experience the portion of the throughput graph that lies above steady-state? Given the distance to the downstream intersection, what is the optimal timing plan to preclude significant congestion effects?

%From the length of the queue and shape of throughput curve, can the optimal cycle duration be derived? 










==> 2 - Copy/intro.tex <==
The capacity of a freeway will increase if vehicles traveling at the speed limit could do so at much shorter
headway, since the flow is just the product of speed and density, which is just the inverse of the
headway.  Adaptive cruise control (ACC) and cooperative adaptive cruise control (CACC) are longitudinal control
technologies that permit headway reduction by a factor of 2 or 3 (compared with manual driving), and thereby increasing freeway capacity by the same factor.  A group of vehicles traveling with short headway is called a platoon.  The earliest  demonstration of
an 8-car platoon of vehicles traveling 16 feet apart at 60 mph, 
was conducted on the I-15 freeway in San Diego in August 1997 (\cite{NAHSRC, shladover-keynote}).  Several other demonstrations have  been
carried out since then, e.g. (\cite{ploeg, cacc-milanes}).  These demonstrations show that headway reduction by a factor of 2 to 3 can be achieved today.

However, increasing the capacity of urban roads by platooning would not increase the throughput of an urban road network whose bottlenecks occur at intersections. For example,   In a standard intersection with 4 approaches and two lanes--one through  and one left-turn lane each with
a capacity of 2000 vph(vehicles per hour) --the total capacity of the roads leading to the intersection is $8 \times 2000 = 16,000$vph .  But the intersection can accommodate only two movements safely at the same time, hence the intersection's capacity is only 4,000 vph or 25 percent of the road capacity.  So increasing the latter
capacity by platooning will do nothing to increase the capacity of the road network.

This observation is at the core of the remarkable study \cite{platoons} to increase the throughput or saturation flow rate of an intersection by having
cars cross the intersection in a platoon of ACC or CACC vehicles. The study concludes: if the saturation flow rates at all intersections in an urban network is increased by a factor $\G$, ``the network can support an increase in demand by the same factor $\G$, with no increase in queuing delay or travel time, and using the same signal control. However, the queues will also grow by the same factor $\G$, so if this leads to a saturation of the links, the improvement in throughput will be sub-linear in $\G$. On the other hand, if the cycle time is reduced, the queues will also be reduced, and this may restore the linear growth in demand.''

The authors stress two limitations of their study, which this paper overcomes.  First, the study assumes that there is a 100 percent penetration of (C)ACC vehicles, whereas the present paper studies the effect of an arbitrary proportion of manual, CC and ACC vehicles.  (The effect on freeway capacity of such
arbitrary proportions is evaluated in \cite{mahmaCVT}.)  ``The second limitation is that in short urban links vehicles will slow down quickly as queues build up. As a result the saturation flow rate at the upstream intersection will be reduced, thereby depriving the system of the full productivity benefit. It is important to investigate this reduction.'' That investigation is carried out in this paper.

Our investigation is carried out on the basis of simulaton results using the Improved Intelligent Driver Model \cite{treiberkesting_book} or IIDM in SUMO.  IIDM
improves upon the IDM model \cite{treiberetal2000} by eliminating some of the latter's unrealistic behaviors. IIDM is reviewed in Section~\ref{sec_cfmrev1}. In 
Section~\ref{sec_intersection_throughput} we discuss intersection throughput for manually driven vehicles, and in Section~\ref{sec_acc_caccrev1}, 
we investigate the increase in  throughput due to (C)ACC.  In Section~\ref{sec_platoon_experimentrev1} we introduce the platoon model
and evaluate ACC and CACC in terms of travel time and network throughput using SUMO simulation~\cite{sumo} of the 4-mile stretch of Colorado Boulevard
/ Huntington Drive arterial with 13 signalized intersections in Arcadia, Southern California. Section~\ref{sec_conclusionrev1} concludes the paper.



==> 2 - Copy/micro_macro.tex <==
Macroscopic models describe traffic in terms of density, and speed.
The road is divided into $1, \dots, N$ links, and the state of
the system at time $t$ is given by the density-speed pair
$\{\rho_i(t), V_i(t)\}_1^N$.
Table~\ref{tab-macro-notation} contains the notation used in macro-modeling. 
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
Symbol & Description & Default value\\
\hline
$\Delta x_i$ & Length of link $i$. & $\Delta x_i = 5$ m.\\
$t$, $\Delta t$ & Time and the model time step
(same as in the car following model). & $\Delta t = 0.05$ s.\\
$\rho_i(t)$ & Vehicle density in link $i$. & \\
$\rho_J$ & Maximal admissible (jam) density. & $\rho_J=1/9$ veh. per meter.\\
$V_i(t)$ & Average traffic speed link $i$. &\\
$v_{\max}$ & Maximal admissible traffic speed
(same as in the car following model). & $v_{\max}=20$ m/s.\\
$f_i(t)$ & Vehicle flow out of link $i$. &\\
$f_0(t)$ & Vehicle flow entering link $1$. &\\
\hline
\end{tabular}
\end{center}
\caption{Macro-modeling notation.}
\label{tab-macro-notation}
\end{table}

Vehicle density $\rho_it)$ is computed from the gap between vehicles and the
vehicle length:
\be
\rho_i(t) = \frac{1}{g_i(t) + l},
\label{eq_mmr_rho}
\ee
where notation $g_i(t)$ defines average gap between vehicles that are
in link $i$ at time $t$.
Obviously, $\rho_i(t)\leq\rho_J = \frac{1}{g_{\min}+l}$.

Every time step, density values in each link are updated according
to the conservation law:
\be
\rho(t+\Delta t) = \rho_i(t) + \frac{\Delta t}{\Delta x_i}\left(f_{i-1}(t) - f_i(t)\right), \;\;\;
i = 1,\dots,N,
\label{eq_macro_rho}
\ee
where $f_i(t) = \rho_i(t)V_i(t)$,
and the entering flow $f_0(t)$ is given.

The speed equation is derived from vehicle speed.
For points $(t, x)$ on the trajectory of a vehicle,
we can write:
\[ v(t) = V(t, x) .\]
The change in position during one time step $\Delta t$ can be expressed
by the first order Taylor expansion around $(t, x)$:
\begin{eqnarray*}
v(t+\Delta t) & = & V(t+\Delta t, x+v(t)\Delta t) \\
& = & V(t, x) + \frac{\partial V(t, x)}{\partial t}\Delta t +
\frac{\partial V(t, x)}{\partial x}v(t)\Delta t \\
& = & V(t, x) + \left(\frac{\partial V}{\partial t} + V(t,x)\frac{\partial V}{\partial x}\right)\Delta t.
\end{eqnarray*}
At the same time, from the car following model we have:
\[ v(t + \Delta t) = v(t) + a(t)\Delta t .\]
Thus, we get:
\[ V(t, x) + \left(\frac{\partial V}{\partial t} +
V(t,x)\frac{\partial V}{\partial x}\right)\Delta t =
V(t, x) + a(t)\Delta t, \]
which, after cancelling $V(t, x)$ and dividing both sides of the equation
by $\Delta t$, yields:
\[\frac{\partial V}{\partial t} + V(t,x)\frac{\partial V}{\partial x} = a(t).\]
Discretizing this equation in time and space, we can write:
\[ \frac{V_i(t+\Delta) - V_i(t)}{\Delta t} +
V_i(t) \frac{V_i(t)-V_{i-1}(t)}{\Delta x_i} = a_i(t) , \;\;\; i=1,\dots,N, \]
and $V_0(t) = V_1(t)$.

Thus, we obtain the speed equation:
\be
V_i(t+\Delta t) = V(t) +
\left(a_i(t) - V_i(t)\frac{V_i(t)-V_{i-1}(t)}{\Delta x_i}\right)\Delta t.
\label{eq_macro_speed}
\ee

Here $a_i(t)$ is defined by the car following model.
\begin{itemize}
\item For Gipps model, following~\eqref{eq_gipps}, we have:
\be
a_i(t) = \min\left\{a_{\max}, \frac{v_{\max}-V_i(t)}{\Delta t}, 
\frac{-V_i(t) - b\tau
+ \sqrt{(b\tau)^2 + (V_{i+1}(t))^2 +
2b\left(\frac{1}{\rho_i(t)}-\frac{1}{\rho_J}\right)}}{\Delta t}\right\},
\label{eq_macro_gipps}
\ee
$i=1,\dots,N$; $V_{N+1}=v_{\max}$.
\item For IIDM, following~\eqref{eq_iidm}, we have:
\be
a_i(t) = \left\{\begin{array}{ll}
a_{\max}\left(1 - \frac{g_{d,i}(t)}{g_i(t)}\right), &
\mbox{ if } \frac{g_{d,i}(t)}{g_i(t)} \geq 1,\\
a_i^\ast(t)\left(1 - \left(\frac{g_{d,i}(t)}{g_i(t)}
\right)^{\delta_1 a_{\max}/a_i^\ast(t)}
\right), & \mbox{ otherwise},
\end{array}\right. 
\label{eq_macro_iidm0}
\ee
where
\be
a_i^\ast(t) =
a_{\max}\left(1-\left(\frac{V_i(t)}{v_{\max}}\right)^{\delta_2}\right),
\label{eq_macro_iidm_afree}
\ee
while the actual gap, $g_i(t)$, and the desired gap,
$g_{d,i}(t)$, can be expressed through density:
\be
g_i(t) = \frac{1}{\rho_i(t)}-l, \;\;\; i=1,\dots,N,
\label{eq_macro_iidm_gap}
\ee
and
\be
g_{d,i}(t) = \frac{1}{\rho_J}-l + \max\left\{0,
V_i(t)\tau + \frac{V_i(t)(V_i(t)-V_{i+1}(t))}{2\sqrt{a_{\max}b}}\right\}, \;\;
i=1,\dots,N; \;\; V_{N+1}=v_{\max}. 
\label{eq_macro_iidm_desired_gap}
\ee
\item For Helly model, following~\eqref{eq_helly}, we have:
\be
a_i(t) = \min\left\{a_{\max}, \frac{v_{\max}-V_i(t)}{\Delta t}, 
\alpha_1\left(V_{i+1}(t)-V_i(t)\right) + 
\alpha_2\left(\frac{1}{\rho_i(t)}-\frac{1}{\rho_J}-V_i(t)\tau\right)\right\},
\label{eq_macro_helly}
\ee
$i=1,\dots,N$; $V_{N+1}=v_{\max}$.
\end{itemize}


\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/macro_contours.png}
\caption{Flow (top) and speed (bottom) contours generated by the
IIDM-induced macroscopic
model in the experiment with the red light downstream for
$a_{\max} = 0.8$, $1.5$ and $2.5\mbox{ m/s}^2$.}
\label{fig-macro-contours}
\end{figure}

As an example,
we reproduced the experiment with the red light ahead and the red light
at the second intersection in the macroscopic environment.
The road is split into 240 links, each with length $l=5$ meters.
The first signal is located at link 50.
The initial condition is:
\begin{eqnarray*}
& & \rho_i(0) = \rho_J = \frac{1}{g_{\min}+l} = \frac{1}{4+5} =1/9, \;\;\; 1=1,\dots,49; \\
& & \rho_i(0) = 0, \;\;\; i = 50,\dots,N=240; \\
& & V_i(0) = 0, \;\;\; i = 1,\dots,N=240.
\end{eqnarray*}
The second signal with the red light is in link 110 (300 meters downstream of
the first one), which translates into condition:
\[ f_{110}(\cdot) = 0. \]

Figure~\ref{fig-macro-contours} presents the flow and speed contours,
produced by the simulation of 60 seconds of the IIDM-induced macroscopic model
for $a_{\max}=0.8, 1.5$ and $2.5\mbox{ m/s}^2$.
Here, the horizontal axis represents time in seconds and
the vertical axis --- space in meters, where cars travel from bottom to top.
The locations of the first and the second signals are at positions 0 and 300
on the vertical axis respectively.



==> 2 - Copy/platoon_experiment.tex <==
Vehicles equipped with CACC can form platoons. 
With 50\% CACC penetration rate, platoons provide between 24 and 44\%
increase in intersection throughput on average, depending on the proximity
of intersections.

In simulation, platoon management and formation is divided into three phases:
1) Identifying vehicles that can be grouped into platoons;
2) Adjusting parameters of leaders and followers in platoons;
3) performing maintenance on the platoon.
This behavior is modeled by the state machine in Fig.~\ref{fig-state-machine}.

\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/state_machine.pdf}
\caption{State machine of a platoon vehicle.}
\label{fig-state-machine}
\end{figure}

To form a platoon, vehicles must be in sequence
with one another on a given lane.
However, vehicles need not share the same final destination
and are free to switch lanes or leave the platoon if necessary.
If an intermediate vehicle in the platoon changes its route by
making a turn or changing lanes, the platoon splits into two:
one platoon for the vehicles ahead of the intermediate vehicle
and another for all the vehicles behind.

A platoon's lead vehicle has the same properties as ACC vehicles.
An isolated CACC vehicle is a leader of a platoon of size 1.
When a platoon leader comes into range of another CACC vehicle in front,
it joins the platoon becoming a follower.
Followers have reduced headway and travel much closer to one another
than standalone vehicles.
In addition, followers are able to receive information from the leader,
such as to accelerate after a green light at an intersection or to
decelerate approaching an obstacle, e.g. red light, downstream.

Since followers are not bound to the same route as the platoon leader,
they are free to separate.
After leaving the platoon, the headway and acceleration parameters are
restored to their original values.
This can happen for example when the follower changes its route or
becomes separated from the rest of platoon, e.g., due to switching
traffic signal as it crosses the intersection.

To study the impact of platooning, we used a SUMO model of the
4-mile stretch of Colorado Boulevard / Huntington Drive arterial
with 13 signalized intersections in Arcadia, Southern California,
shown in Fig.~\ref{fig-huntcol}.
IIDM and CACC models were implemented in SUMO, and platoon management
and formation were handled via SUMO/TraCI API.
Using real world flow measurements and estimated turn ratios at intersections,
we generated 1 hour  of origin-destination (OD) travel demand data.
\begin{figure}[h]
\centering
\includegraphics[width=3.2in]{figures/huntcol_gmaps.png}
\caption{Huntington Colorado network modeled in SUMO.}
\label{fig-huntcol}
\end{figure}
Then, we ran a series of simulation varying the fraction of ACC (CACC) vehicles
from 0 to 75\%.
In each simulation two vehicle classes were modeled: ordinary vehicles
and ACC (or CACC) vehicles.
In simulations with CACC vehicles platoons were formed.
The total number of OD pairs in this network is 399.
The same number of vehicles was processed in each simulation.
The rates and locations at which cars were generated were identical
in all scenarios to eliminate the variance in randomly generated routes.
For  cases of 0, 25, 50 and 75 percent  ACC (CACC) penetration rate,
we computed average travel time for the route O$\rightarrow$D, where O and D
identify origin and destination of the  selected west-east route
in Fig.~\ref{fig-huntcol}.
Table~\ref{tab-timesIIDM} lists the mean
travel time (MTT) and its standard deviation (STD),  in seconds.  As expected,
the mean travel time reduces as the fraction of (C)ACC vehicles increases.  Surprisingly the standard deviation also decreases.  Furthermore, the travel time of ordinary vehicles
is also reduced, although that of (C)ACC vehicles is reduced more.

\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
[C]ACC & Vehicle & \multicolumn{2}{|c|}{ACC} & \multicolumn{2}{|c|}{CACC} \\
\cline{3-6}
\% & Class & MTT & STD & MTT & STD \\
\cline{1-6}
0 & ordinary & 653 & 102 & 653 & 102 \\
\cline{1-6}
\multirow{3}{*}{25\%} & ordinary & 640 & 96 & 638 & 96 \\
 & [C]ACC & 605 & 82 & 600 & 76 \\
 & all & 631 & 94 & 629 & 94\\
\cline{1-6}
\multirow{3}{*}{50\%} & ordinary & 583 & 66 & 579 & 60 \\
 & [C]ACC & 583 & 61 & 570 & 64 \\
 & all & 583 & 64 & 575 & 62\\
\cline{1-6}
\multirow{3}{*}{75\%} & ordinary & 595 & 45 & 583 & 41\\
 & [C]ACC & 558 & 58 & 540 & 52\\
 & all & 567 & 57 & 550 & 48\\
\cline{1-6}
\end{tabular}
\caption{Mean travel time (MTT) and standard deviation (STD) in seconds for varying percentage of ACC vehicles on the main arterial of Fig.~\ref{fig-huntcol}.}
\label{tab-timesIIDM}
\end{table}



==> 2 - Copy/platoon_model.tex <==

Platoon management entails three general phases: 1) Identifying vehicles that can be grouped into platoons. 2) Setting individual platoon speed advisories to maximize flow. 3) Performing maintenance on the current platoon. 

At a minimum, platoons must be in a contigeous location on a given lane. During designated platoon formation phases, each lane is processed individually, and any ACC vehicles in sequence are combined into a platoon. There is no requirement that vehicles within any given platoon have the same route or same following turn. Vehicles still perform in their own best interest, so they are not restricted from switching lanes and leaving the platoon if they individually decide it is optimal.

All non-leading vehicles have both their gap parameters reduced to the platoon values. In order to maintain safe distances within platoons, the leading car constantly monitors the speed of the vehicle ahead of it, along with the current headway. As soon as it is forced to decelerate due to a decreasing headway, it propagates the message to the rest of the vehicles in the platoons to also decelerate the same amount. 

At designated time steps, platoons are processed to check validity. Whenever a vehicle switches lane or makes a turn that is not in line with the rest of the platoon, it is immediately removed and its parameters are restored to regular ACC values. A platoon is forced to divide if a traffic signal switches as it is crossing the intersection or if a non-ACC vehicle enters in between two vehicles in the platoon. In all situations, the rear portion of the platoon forms a new separate platoon and the new leader's parameters are restored to regular ACC values. This process allows for a seamless update of platoon states without causing deceleration in the platoon overall.

Figure~\ref{fig-sm}. Finite Automata describing platoon behavior. [illustrator version in folder]

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/state_machine.jpg}
\caption{State machine describing vehicle behavior in the platoon.}
\label{fig-sm}
\end{figure}

This procedure allowed for a further increase in throughput of approximately X percent along the main arterial roads; Huntington and Colorado.



==> iidm_boxplot.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
unbounded coords=jump,
xmin=0.5,
xmax=4.5,
xtick={1,2,3,4},
xticklabels={{0},{25},{50},{75}},
ymin=340.16,
ymax=3588.24,
axis background/.style={fill=white}
]
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	3042.5\\
1	3440.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	2414.4\\
2	2712.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	1976.85\\
3	2212.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	1365.45\\
4	1556.3\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	694.3\\
1	1593.1\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	653.9\\
2	1440.55\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	625.7\\
3	1206.4\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	487.8\\
4	798.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	3440.6\\
1.125	3440.6\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	2712.3\\
2.125	2712.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	2212.3\\
3.125	2212.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	1556.3\\
4.125	1556.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	694.3\\
1.125	694.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	653.9\\
2.125	653.9\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	625.7\\
3.125	625.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	487.8\\
4.125	487.8\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.75	1593.1\\
0.75	3042.5\\
1.25	3042.5\\
1.25	1593.1\\
0.75	1593.1\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
1.75	1440.55\\
1.75	2414.4\\
2.25	2414.4\\
2.25	1440.55\\
1.75	1440.55\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
2.75	1206.4\\
2.75	1976.85\\
3.25	1976.85\\
3.25	1206.4\\
2.75	1206.4\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
3.75	798.7\\
3.75	1365.45\\
4.25	1365.45\\
4.25	798.7\\
3.75	798.7\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.75	2406.3\\
1.25	2406.3\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
1.75	2008.5\\
2.25	2008.5\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
2.75	1584.7\\
3.25	1584.7\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
3.75	1106.7\\
4.25	1106.7\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\end{axis}
\end{tikzpicture}%

==> iidm_boxplot_npltn.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
unbounded coords=jump,
xmin=0.5,
xmax=4.5,
xtick={1,2,3,4},
xticklabels={{0},{25},{50},{75}},
ymin=370.82,
ymax=3586.78,
axis background/.style={fill=white}
]
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	3042.5\\
1	3440.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	2653.75\\
2	2901.8\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	1978.85\\
3	2355.5\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	1590.6\\
4	1751.7\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
1	694.3\\
1	1593.1\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
2	642.1\\
2	1457.6\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
3	517\\
3	1218.15\\
};
\addplot [color=black,dashed,forget plot]
  table[row sep=crcr]{%
4	547.2\\
4	895.1\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	3440.6\\
1.125	3440.6\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	2901.8\\
2.125	2901.8\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	2355.5\\
3.125	2355.5\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	1751.7\\
4.125	1751.7\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
0.875	694.3\\
1.125	694.3\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
1.875	642.1\\
2.125	642.1\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
2.875	517\\
3.125	517\\
};
\addplot [color=black,solid,forget plot]
  table[row sep=crcr]{%
3.875	547.2\\
4.125	547.2\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
0.75	1593.1\\
0.75	3042.5\\
1.25	3042.5\\
1.25	1593.1\\
0.75	1593.1\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
1.75	1457.6\\
1.75	2653.75\\
2.25	2653.75\\
2.25	1457.6\\
1.75	1457.6\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
2.75	1218.15\\
2.75	1978.85\\
3.25	1978.85\\
3.25	1218.15\\
2.75	1218.15\\
};
\addplot [color=blue,solid,forget plot]
  table[row sep=crcr]{%
3.75	895.1\\
3.75	1590.6\\
4.25	1590.6\\
4.25	895.1\\
3.75	895.1\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
0.75	2406.3\\
1.25	2406.3\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
1.75	2085.8\\
2.25	2085.8\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
2.75	1628.75\\
3.25	1628.75\\
};
\addplot [color=red,solid,forget plot]
  table[row sep=crcr]{%
3.75	1201.05\\
4.25	1201.05\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\addplot [color=black,only marks,mark=+,mark options={solid,draw=red},forget plot]
  table[row sep=crcr]{%
nan	nan\\
};
\end{axis}
\end{tikzpicture}%

==> intersection_throughput.tex <==


\subsection{Baic Experiment: Single Intersection}\label{subsec_basic}




\subsection{Effect of the Downstream Queue}\label{subsec_queue_effect}








For vehicles traveling at constant speed with a uniform space headway, the observed throughput per hour is inversely proportional to the reaction time. In particular, for vehicles moving at 20 m/s and a reaction time of 2.5 s (equivalent to a space headway of 2.5 $\times$ 20 = 50 m), a saturation flow rate of 3600/2.5 = 1440 vph is achieved, hereinafter referred to as the steady-state throughput. (cite platoons of connected vehicles... varaiya 2015) \\

With the introduction of a traffic signal and the build-up of a large queue of vehicles, the instantaneous throughput of vehicles can be measured by recording the time headway between successive vehicles. For a sufficiently long green signal in the outbound direction, the time headway of the vehicles is expected to converge to the steady-state equilibrium and the steady-state throughput is believed to be an upper bound on the total flow achievable. However, in simulation it was observed that the total throughput in fact exceeded the steady-state throughput. This was contingent on factors that the steady-state calculations do not consider, such as the rate of acceleration and deceleration of the vehicles. When the signal turns green, the first few cars are packed together due to their accelerating behavior and are not as widely spaced as the cars further in the queue when they approach the intersection. As a result, the observed time headway is less than the steady-state reaction time and an increased throughput is observed.\\

Different scenarios were considered with varying accelerations as well as varying red clear times between switching green signals. The instantaneous throughput for each scenario was plotted and compared to the steady-state theoretical. 


\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/init.jpg}
\caption{Simulation set up with large queues in the North and West lanes both traveling East.}
\label{fig:init}
\end{figure}

Figure \ref{fig:init} shows a picture of the simulation in SUMO. The parameters used were $\theta_{\min} = 2.5$ s with $g_{\min} = 4$ m, $l = 5$ m, $v_{\max} = 20$ m/s, and $\tau = 2.05$ s.  

The first parameter investigated was the affect of signal length. Two different signal plans were used: a one minute cycle and a two minute cycle, each with identical red clear times. For example, a three second red clear time for a two minute cycle would result in the following signal pattern: 57 seconds of EW green, 3 second of all red, 57 seconds of NS green and 3 seconds of all red. This implies that for a one minute cycle, double the red clear time is experienced compared to the two minute cycle for simulations that are integer multiples of two minutes in length. 

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_a15.png}
\caption{Comparison of timing plans for the scenario highlighted in Figure \ref{fig:init} with a red clear time of 3 seconds and acceleration equal to $1.5$ m/s$^2$. The troughs in the curves represent the transition between the last car from the East and the first car in the North and vice versa.}
\label{fig:cycles}
\end{figure}


Although a total decrease in throughput is expected for the one minute cycle, the total throughput in both scenarios highlighted in figure \ref{fig:cycles} was 1440 vehicles after one hour of simulation. This indicates the loss in throughput experienced by more frequently changing timing plans (and consequently more troughs) was balanced out by the high throughput experienced initially after the signal turned green in each direction. Despite this, the total throughput experienced after one hour was equivalent to the steady-state throughput. With a red clear time of 0 seconds, the total throughput observed for the same scenarios were \textbf{ XXXXXXXXXXX} for the one minute and two minute cycles respectively. This implies, paradoxically, that the introduction of a traffic signal in the presence of a seemingly infinite queue can increase the throughput beyond the steady-state bound. \\


The next parameter examined was the maximum acceleration of the vehicles. For vehicles that were not at the front of the queue, their speeds were dictated by (3) whereas the speed of the vehicle at the front of the queue was governed by simple kinematics: $v(t+\Delta t) = v(t) + a\Delta t$ \textbf{(not sure how to cross reference between tex files for equations)} Consequently, the acceleration of the lead vehicle was directly correlated with the speed of its followers - a larger acceleration implied that the following vehicles were able to travel faster as well. As a result, the instantaneous throughput and total throughput observed were larger for the scenarios with higher accelerations. Figure \ref{fig:diffa} compares varying accelerations and the resulting throughputs.\\

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_diffa.png}
\caption{Comparison of accelerations for the scenario highlighted in Figure \ref{fig:init} with a red clear time of 3 seconds and a two minute cycle. The total throughput after one hour for $a = 1.0,\  1.5,\  2.6$ m/s$^2$ was 1380, 1440 and 1510 vehicles respectively.}
\label{fig:diffa}
\end{figure}



Finally, the duration of the red clear time was also experimented with. Increasing the red clear time would predictably decrease the total throughput and increase the size of the troughs in the throughput plots. 

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/manual_diffRCT.png}
\caption{Comparison of red clear times for the scenario highlighted in Figure \ref{fig:init} with a two minute cycle.}
\label{fig:diffRCT}
\end{figure}

In Figure \ref{fig:diffRCT} it is clear that the decrease in throughput between a red clear time of 0 seconds and 3 seconds is much larger than that between 3 seconds and 5 seconds.\\

Although this provides insight into the dynamics of the cars, it is an idealized scenario. As in most urban settings, there is often another signal further downstream, leading to the formation of another queue between the two intersections. This congestion effect significantly decreases the throughput through the first intersection and is correlated with the distance between the two intersections. Figures \ref{fig:100m} and \ref{fig:500m} plot the instantaneous throughput through the first intersection in the presence of a downstream intersection that is 100m and 500m away respectively. The timing plan of the second intersection flipped the order of the green waves. Although the order of the second timing plan is arbitrary, the total throughput will be the same.\\

\textbf{(not sure if graph for 100m is totally correct - had teleporting issues, cite source about how long between intersections in urban setting)}

\begin{figure}[htb!]
\centering
\includegraphics[width=5in]{figures/100m.png}
\caption{Throughput in the presence of downstream intersection 100m away.}
\label{fig:100m}
\end{figure}

\begin{figure}[htb!]
\centering
\includegraphics[width=5in]{figures/500m.png}
\caption{Throughput in the presence of downstream intersection 500m away.}
\label{fig:500m}
\end{figure}

For the 100m and 500m downstream intersections, the total throughput after an hour was 753 and 772 vehicles for zero seconds of red clear time and 722 and 742 vehicles for three seconds of red clear time respectively. For the secondary intersection 100m away, although the peak is much closer to the steady-state theoretical compared to the 500m scenario, its trough is much larger. Because of this, the throughput experienced on average for the 500m scenario is in fact larger as is expected. 

%\begin{figure}
%\centering
%\begin{minipage}{.7\textwidth}
%  \centering
%  \includegraphics[width=.8\linewidth]{figures/100m.png}
%  \captionof{figure}{A figure}
%  \label{fig:test1}
%\end{minipage}%
%\begin{minipage}{.7\textwidth}
%  \centering
%  \includegraphics[width=.8\linewidth]{figures/500m.png}
%  \captionof{figure}{Another figure}
%  \label{fig:test2}
%\end{minipage}
%\end{figure}


This, in conjunction with the results of varying acceleration and timing plans, poses further questions: for a given acceleration, what is the optimal signal length and red clear time to maximize the number of cars that can pass through an intersection? Is it more advantageous to have short bursts in cycles to solely experience the portion of the throughput graph that lies above steady-state? Given the distance to the downstream intersection, what is the optimal timing plan to preclude significant congestion effects?

%From the length of the queue and shape of throughput curve, can the optimal cycle duration be derived? 










==> micro_macro.tex <==
Macroscopic models describe traffic in terms of density, and speed.
The road is divided into $1, \dots, N$ links, and the state of
the system at time $t$ is given by the density-speed pair
$\{\rho_i(t), V_i(t)\}_1^N$.
Table~\ref{tab-macro-notation} contains the notation used in macro-modeling. 
\begin{table}[h]
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
Symbol & Description & Default value\\
\hline
$\Delta x_i$ & Length of link $i$. & $\Delta x_i = 5$ m.\\
$t$, $\Delta t$ & Time and the model time step
(same as in the car following model). & $\Delta t = 0.05$ s.\\
$\rho_i(t)$ & Vehicle density in link $i$. & \\
$\rho_J$ & Maximal admissible (jam) density. & $\rho_J=1/9$ veh. per meter.\\
$V_i(t)$ & Average traffic speed link $i$. &\\
$v_{\max}$ & Maximal admissible traffic speed
(same as in the car following model). & $v_{\max}=20$ m/s.\\
$f_i(t)$ & Vehicle flow out of link $i$. &\\
$f_0(t)$ & Vehicle flow entering link $1$. &\\
\hline
\end{tabular}
\end{center}
\caption{Macro-modeling notation.}
\label{tab-macro-notation}
\end{table}

Vehicle density $\rho_it)$ is computed from the gap between vehicles and the
vehicle length:
\be
\rho_i(t) = \frac{1}{g_i(t) + l},
\label{eq_mmr_rho}
\ee
where notation $g_i(t)$ defines average gap between vehicles that are
in link $i$ at time $t$.
Obviously, $\rho_i(t)\leq\rho_J = \frac{1}{g_{\min}+l}$.

Every time step, density values in each link are updated according
to the conservation law:
\be
\rho(t+\Delta t) = \rho_i(t) + \frac{\Delta t}{\Delta x_i}\left(f_{i-1}(t) - f_i(t)\right), \;\;\;
i = 1,\dots,N,
\label{eq_macro_rho}
\ee
where $f_i(t) = \rho_i(t)V_i(t)$,
and the entering flow $f_0(t)$ is given.

The speed equation is derived from vehicle speed.
For points $(t, x)$ on the trajectory of a vehicle,
we can write:
\[ v(t) = V(t, x) .\]
The change in position during one time step $\Delta t$ can be expressed
by the first order Taylor expansion around $(t, x)$:
\begin{eqnarray*}
v(t+\Delta t) & = & V(t+\Delta t, x+v(t)\Delta t) \\
& = & V(t, x) + \frac{\partial V(t, x)}{\partial t}\Delta t +
\frac{\partial V(t, x)}{\partial x}v(t)\Delta t \\
& = & V(t, x) + \left(\frac{\partial V}{\partial t} + V(t,x)\frac{\partial V}{\partial x}\right)\Delta t.
\end{eqnarray*}
At the same time, from the car following model we have:
\[ v(t + \Delta t) = v(t) + a(t)\Delta t .\]
Thus, we get:
\[ V(t, x) + \left(\frac{\partial V}{\partial t} +
V(t,x)\frac{\partial V}{\partial x}\right)\Delta t =
V(t, x) + a(t)\Delta t, \]
which, after cancelling $V(t, x)$ and dividing both sides of the equation
by $\Delta t$, yields:
\[\frac{\partial V}{\partial t} + V(t,x)\frac{\partial V}{\partial x} = a(t).\]
Discretizing this equation in time and space, we can write:
\[ \frac{V_i(t+\Delta) - V_i(t)}{\Delta t} +
V_i(t) \frac{V_i(t)-V_{i-1}(t)}{\Delta x_i} = a_i(t) , \;\;\; i=1,\dots,N, \]
and $V_0(t) = V_1(t)$.

Thus, we obtain the speed equation:
\be
V_i(t+\Delta t) = V(t) +
\left(a_i(t) - V_i(t)\frac{V_i(t)-V_{i-1}(t)}{\Delta x_i}\right)\Delta t.
\label{eq_macro_speed}
\ee

Here $a_i(t)$ is defined by the car following model.
\begin{itemize}
\item For Gipps model, following~\eqref{eq_gipps}, we have:
\be
a_i(t) = \min\left\{a_{\max}, \frac{v_{\max}-V_i(t)}{\Delta t}, 
\frac{-V_i(t) - b\tau
+ \sqrt{(b\tau)^2 + (V_{i+1}(t))^2 +
2b\left(\frac{1}{\rho_i(t)}-\frac{1}{\rho_J}\right)}}{\Delta t}\right\},
\label{eq_macro_gipps}
\ee
$i=1,\dots,N$; $V_{N+1}=v_{\max}$.
\item For IIDM, following~\eqref{eq_iidm}, we have:
\be
a_i(t) = \left\{\begin{array}{ll}
a_{\max}\left(1 - \frac{g_{d,i}(t)}{g_i(t)}\right), &
\mbox{ if } \frac{g_{d,i}(t)}{g_i(t)} \geq 1,\\
a_i^\ast(t)\left(1 - \left(\frac{g_{d,i}(t)}{g_i(t)}
\right)^{\delta_1 a_{\max}/a_i^\ast(t)}
\right), & \mbox{ otherwise},
\end{array}\right. 
\label{eq_macro_iidm0}
\ee
where
\be
a_i^\ast(t) =
a_{\max}\left(1-\left(\frac{V_i(t)}{v_{\max}}\right)^{\delta_2}\right),
\label{eq_macro_iidm_afree}
\ee
while the actual gap, $g_i(t)$, and the desired gap,
$g_{d,i}(t)$, can be expressed through density:
\be
g_i(t) = \frac{1}{\rho_i(t)}-l, \;\;\; i=1,\dots,N,
\label{eq_macro_iidm_gap}
\ee
and
\be
g_{d,i}(t) = \frac{1}{\rho_J}-l + \max\left\{0,
V_i(t)\tau + \frac{V_i(t)(V_i(t)-V_{i+1}(t))}{2\sqrt{a_{\max}b}}\right\}, \;\;
i=1,\dots,N; \;\; V_{N+1}=v_{\max}. 
\label{eq_macro_iidm_desired_gap}
\ee
\item For Helly model, following~\eqref{eq_helly}, we have:
\be
a_i(t) = \min\left\{a_{\max}, \frac{v_{\max}-V_i(t)}{\Delta t}, 
\alpha_1\left(V_{i+1}(t)-V_i(t)\right) + 
\alpha_2\left(\frac{1}{\rho_i(t)}-\frac{1}{\rho_J}-V_i(t)\tau\right)\right\},
\label{eq_macro_helly}
\ee
$i=1,\dots,N$; $V_{N+1}=v_{\max}$.
\end{itemize}


\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/macro_contours.png}
\caption{Flow (top) and speed (bottom) contours generated by the
IIDM-induced macroscopic
model in the experiment with the red light downstream for
$a_{\max} = 0.8$, $1.5$ and $2.5\mbox{ m/s}^2$.}
\label{fig-macro-contours}
\end{figure}

As an example,
we reproduced the experiment with the red light ahead and the red light
at the second intersection in the macroscopic environment.
The road is split into 240 links, each with length $l=5$ meters.
The first signal is located at link 50.
The initial condition is:
\begin{eqnarray*}
& & \rho_i(0) = \rho_J = \frac{1}{g_{\min}+l} = \frac{1}{4+5} =1/9, \;\;\; 1=1,\dots,49; \\
& & \rho_i(0) = 0, \;\;\; i = 50,\dots,N=240; \\
& & V_i(0) = 0, \;\;\; i = 1,\dots,N=240.
\end{eqnarray*}
The second signal with the red light is in link 110 (300 meters downstream of
the first one), which translates into condition:
\[ f_{110}(\cdot) = 0. \]

Figure~\ref{fig-macro-contours} presents the flow and speed contours,
produced by the simulation of 60 seconds of the IIDM-induced macroscopic model
for $a_{\max}=0.8, 1.5$ and $2.5\mbox{ m/s}^2$.
Here, the horizontal axis represents time in seconds and
the vertical axis --- space in meters, where cars travel from bottom to top.
The locations of the first and the second signals are at positions 0 and 300
on the vertical axis respectively.



==> platoon_model.tex <==

Platoon management entails three general phases: 1) Identifying vehicles that can be grouped into platoons. 2) Setting individual platoon speed advisories to maximize flow. 3) Performing maintenance on the current platoon. 

At a minimum, platoons must be in a contigeous location on a given lane. During designated platoon formation phases, each lane is processed individually, and any ACC vehicles in sequence are combined into a platoon. There is no requirement that vehicles within any given platoon have the same route or same following turn. Vehicles still perform in their own best interest, so they are not restricted from switching lanes and leaving the platoon if they individually decide it is optimal.

All non-leading vehicles have both their gap parameters reduced to the platoon values. In order to maintain safe distances within platoons, the leading car constantly monitors the speed of the vehicle ahead of it, along with the current headway. As soon as it is forced to decelerate due to a decreasing headway, it propagates the message to the rest of the vehicles in the platoons to also decelerate the same amount. 

At designated time steps, platoons are processed to check validity. Whenever a vehicle switches lane or makes a turn that is not in line with the rest of the platoon, it is immediately removed and its parameters are restored to regular ACC values. A platoon is forced to divide if a traffic signal switches as it is crossing the intersection or if a non-ACC vehicle enters in between two vehicles in the platoon. In all situations, the rear portion of the platoon forms a new separate platoon and the new leader's parameters are restored to regular ACC values. This process allows for a seamless update of platoon states without causing deceleration in the platoon overall.

Figure~\ref{fig-sm}. Finite Automata describing platoon behavior. [illustrator version in folder]

\begin{figure}[htb]
\centering
\includegraphics[width=5in]{figures/state_machine.jpg}
\caption{State machine describing vehicle behavior in the platoon.}
\label{fig-sm}
\end{figure}

This procedure allowed for a further increase in throughput of approximately X percent along the main arterial roads; Huntington and Colorado.


